Internal lenses as functors and cofunctors

Lenses may be characterised as objects in the category of algebras over a monad, however they are often understood instead as morphisms, which propagate updates between systems. Working internally to a category with pullbacks, we define lenses as simultaneously functors and cofunctors between categories. We show that lenses may be canonically represented as a particular commuting triangle of functors, and unify the classical state-based lenses with both c-lenses and d-lenses in this framework. This new treatment of lenses leads to considerable simplifications that are important in applications, including a clear interpretation of lens composition.

==> eptcsdata.tex <==
\providecommand{\firstpage}{183}
\providecommand{\publicationstatus}{John Baez and Bob Coecke (Eds.): Applied Category Theory 2019\\
EPTCS 323, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.323.13}{10.4204/EPTCS.323.13}}

